Efficient Answer Enumeration in Description Logics with Functional Roles -- Extended Version

We study the enumeration of answers to ontology-mediated queries when the ontology is formulated in a description logic that supports functional roles and the query is a CQ. In particular, we show that enumeration is possible with linear preprocessing and constant delay when a certain extension of the CQ (pertaining to functional roles) is acyclic and free-connex acyclic. This holds both for complete answers and for partial answers. We provide matching lower bounds for the case where the query is self-join free.

==> cq-fc.tex <==
\section{Partial answers and functionality}
\label{sec:paaf}



\section{Conjunctive queries and functional dependencies}

In \cite{carmeli-enum-func} the authors consider the impact of functional dependencies on the enumeration task
in the setting of plain conjunctive queries. Their main technical result links
the enumeration feasiblity with the structure of so\=/called FD-extended queries.

Let $q$ be a CQ over schema $\Sigma$
and $\Omc$ be a set of functionality assertions of form $\func(R)$,
where $R$ is a role name over $\Sigma$.

Let $\hat{q}$ be a copy of $q$ with every relation symbol $r$ replaced by $\hat{r}$.
Let $\hat{q}(\bar{y})$ be the head of $\hat{q}$.
And let $\hat{\Sigma}$ be a copy of $\Sigma$.

We update $\hat{q}$ and $\hat{\Sigma}$ using the following rules until we achive a fixpoint.
\begin{itemize}
    \item \textbf{Head extension}
    If there is an atom $R(z,z')$ in $q$ such that $\func(R) \in \Omc$ and
    $z \in \bar{y}$ but $z' \notin \bar{y}$, then replace the head of $\hat{q}$ with
    $\hat{q}(\bar{y}z')$.
    \item \textbf{Body extension} If there is an atom $R(z,z')$ in $q$ such that $\func(R) \in \Omc$ and
    there is an atom $\hat{R}(\bar{y}) \in \hat{q}$ such that
    $z \in \bar{y}$ but $z' \notin \bar{y}$, then replace the atom with $\hat{R}(\bar{y}z')$
    and replace every other atom $\hat{R}(\bar{z})$ using the relation symbol $\hat{R}$ with an atom
    $\hat{R}(\bar{z}t_{\bar{z}})$, where $t_{\bar{z}}$ is a fresh variable.
    Update the arity of the symbol $\hat{R} \in \hat{\Sigma}$.
\end{itemize}

The fixpoint of the above operations, called the FD\=/extension of $q$ and denoted $q^+$, exists and is
always achived after a finite number of steps.
Note that the new signature, called $\Sigma^+$, differs from $\Sigma$ and $q^+$ is a CQ over $\Sigma^+$.


The aforementioned link can be expressed as follows.
\begin{theorem}[Theorem 3. in~\cite{carmeli-enum-func}]
    Let $\Sigma$ be a schema,
    let $\Omc$ be a set of functionality assertions of form $\func(R)$, where $R$ is a role name in $\Sigma$.
    If $q^+$ is acyclic and free\=/connec acyclic then enumeration for $q$ is in \emph{in \dlc}.
\end{theorem}

The authors also provide a lower bound that matches the above in the case of CQs
with no self\=/joins.

\begin{lemma}
    \label{lemma:paths-from-q-plus-to-q}
    Let $Q= (\Omc, \Sigma, q)$ be an OMQ.
    For every pair $y,y'$ of distinct variables in $q$, if there is %an atom $\hat{R}(\bar{z}) \in q^+$
%    such that $x,y \in \bar{z}$
    an edge $\{y,y'\}$ in $G_{q^+}$
     then there is a simple path $v_\ell, \dots, v_0, u_0, \dots, u_{\ell'}$ from
     $v_\ell = y$ to $u_{\ell'} = y'$ such that $v_0, \dots, v_\ell$ and $u_0, \dots, u_{\ell'}$
     are simple functional paths.
     %is a simple path $u_0, \dots, u_l$ in $q$
%    from $x=u_0$ to $y=u_l$ such that % for each $0 \leq i < l$ there is an atom $R_i(u_i,u_{i+1}) \in q$, and
%    there is $0\leq j <l$ such that there are a simple functional path from $u_j $ to $x$ and
%    a simple functional path from $u_{j+1} $ to $y$.
\end{lemma}

\begin{proof}
    By definition of the Gaifman graph of $q^+$ there is an atom $\hat{R}(\bar{w})$ in $q^+$
    that uses both $y$ and $y'$. Thus, by construction of $q^+$, there is an atom $R(\bar{z})$
    in $q$ with variables $z,z'$ such that there is a simple functional path $\pi$ from $z$ to $y$
    and a simple functional path $\pi'$ from $z'$ to $y'$.
    Let $x$ be the last variable on $\pi$ that appers in $\pi'$.
    It is easy to check that the concatenation of the paths $\pi$ restricted to path
    from $z$ to $x$ and $\pi'$ restricted to path from $x$ to $z'$ is the desired path.
\end{proof}

